A Meta-Learning Approach to Predicting Performance and Data Requirements

We propose an approach to estimate the number of samples required for a model to reach a target performance. We find that the power law, the de facto principle to estimate model performance, leads to large error when using a small dataset (e.g., 5 samples per class) for extrapolation. This is because the log-performance error against the log-dataset size follows a nonlinear progression in the few-shot regime followed by a linear progression in the high-shot regime. We introduce a novel piecewise power law (PPL) that handles the two data regimes differently. To estimate the parameters of the PPL, we introduce a random forest regressor trained via meta learning that generalizes across classification/detection tasks, ResNet/ViT based architectures, and random/pre-trained initializations. The PPL improves the performance estimation on average by 37% across 16 classification and 33% across 10 detection datasets, compared to the power law. We further extend the PPL to provide a confidence bound and use it to limit the prediction horizon that reduces over-estimation of data by 76% on classification and 91% on detection datasets.

==> tables/data_fewshot.tex <==
\begin{table*}[ht]
\rowcolors{2}{gray!10}{white}
\centering
\caption{Estimating data requirements from few-shot to high-shot for classification tasks.}
\label{T:data_fewshot_classification}
\begin{tabular}{l|rr|rrrr}
\toprule
\multicolumn{7}{c}{CLASSIFICATION}                                                                                                                                                                       \\
\midrule
                    & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7}                    
                    & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
\caltech          & -0.6±0.1                   & -0.1±0.0                   & -0.2±0.2                   & -0.0±0.1                   & -0.0±0.1                       & 3.7±1.9                       \\
\cifar             & inf                        & inf                        & 0.4±0.7                    & 0.5±0.6                    & 0.5±0.6                        & 2.3±1.9                       \\
\cifarh            & 0.2±0.7                    & 0.3±0.6                    & -0.6±0.2                   & 0.0±0.0                    & -0.1±1.2                       & 4.7±0.5                       \\
\cub              & -0.1±0.1                   & -0.1±0.0                   & -0.3±0.0                   & -0.0±0.0                   & -0.0±0.0                       & 4.3±0.9                       \\
\daircraft & inf                        & inf                        & 13.3±11.4                  & 13.3±11.4                  & 0.2±0.0                        & 3.7±0.5                       \\
\ddtd     & 0.7±0.4                    & 0.7±0.4                    & 3.1±1.2                    & 3.1±1.2                    & 1.3±1.3                        & 1.7±0.9                       \\
\dflowers  & -0.0±0.0                   & 0.0±0.0                    & 0.3±0.1                    & 0.3±0.1                    & 0.3±0.1                        & 1.3±0.5                       \\
\ducf  & 18.8±12.4                  & 18.8±12.4                  & 0.6±0.6                    & 0.6±0.5                    & -0.1±0.1                       & 4.7±0.5                       \\
\eurosat             & inf                        & inf                        & -0.7±0.1                   & 0.0±0.1                    & 0.0±0.1                        & 3.3±1.2                       \\
\fgvcaircrafts     & inf                        & inf                        & inf                        & inf                        & 1.0±1.0                        & 2.0±0.8                       \\
\icassava            & 1.7±3.3                    & 1.7±3.3                    & inf                        & inf                        & 0.5±1.4                        & 3.7±1.9                       \\
\mit               & 0.1±0.6                    & 0.3±0.4                    & 0.6±1.2                    & 0.8±1.1                    & 0.1±0.1                        & 3.0±0.8                       \\
\oxfordflowers       & 0.1±0.2                    & 0.2±0.1                    & 0.1±0.2                    & 0.2±0.1                    & 0.2±0.1                        & 2.3±1.9                       \\
\pets                & -0.8±0.0                   & -0.4±0.2                   & -0.8±0.0                   & -0.1±0.0                   & -0.2±0.1                       & 5.0±0.0                       \\
\stanfordcars        & 8.4±1.8                    & 8.4±1.8                    & 15.5±10.2                  & 15.5±10.2                  & 0.2±0.2                        & 3.0±0.0                       \\
\stanforddogs        & -0.3±0.4                   & -0.0±0.2                   & -0.3±0.2                   & -0.1±0.1                   & -0.1±0.0                       & 5.0±0.0                       \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
\rowcolors{2}{gray!10}{white}
\centering
\caption{Estimating data requirements from few-shot to high-shot for detection tasks.}
\label{T:data_fewshot_detection}
\begin{tabular}{l|rr|rrrr}
\toprule
\multicolumn{7}{c}{DETECTION}                                                                                                                                                                            \\
\midrule
                    & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7}                     
                    & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}                    
cityscapes          & 0.4±0.8                    & 0.6±0.7                    & 0.1±0.4                    & 0.4±0.3                    & 0.4±0.3                        & 2.7±1.7                       \\
comic               & inf                        & inf                        & 2.4±2.7                    & 2.7±2.4                    & 2.7±2.5                        & 2.3±1.9                       \\
crowdhuman          & 5.5±7.2                    & 5.5±7.2                    & 1.0±1.5                    & 1.1±1.4                    & 1.1±1.4                        & 1.3±0.5                       \\
duo                 & 1.7±0.7                    & 1.7±0.7                    & 0.8±1.0                    & 0.8±0.9                    & 0.1±0.2                        & 3.3±1.2                       \\
kitti               & 5.0±6.3                    & 5.0±6.3                    & 0.2±0.4                    & 0.4±0.2                    & 0.2±0.2                        & 2.3±1.9                       \\
minneapple          & -0.3±0.7                   & -0.0±0.6                   & -0.6±0.2                   & -0.2±0.2                   & 0.0±0.5                        & 4.3±0.9                       \\
sixray              & 4.0±1.9                    & 4.0±1.9                    & -0.2±0.2                   & -0.0±0.0                   & -0.0±0.0                       & 5.0±0.0                       \\
table               & 0.4±0.7                    & 0.5±0.7                    & 0.6±0.8                    & 0.7±0.7                    & -0.0±0.3                       & 4.3±0.9                       \\
visdrone2019        & 0.0±0.0                    & 0.0±0.0                    & -0.3±0.1                   & -0.1±0.0                   & -0.1±0.0                       & 5.0±0.0                       \\
watercolor          & 6.5±2.9                    & 6.5±2.9                    & 1.9±1.8                    & 1.9±1.7                    & -0.1±0.4                       & 4.0±1.4                      \\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table*}[ht]
% \rowcolors{2}{gray!10}{white}
% \centering
% \caption{Estimating data requirements from few-shot to high-shot}
% \label{T:data_fewshot}
% \begin{tabular}{l|rr|rrrr}
% \toprule
% \multicolumn{7}{c}{CLASSIFICATION}                                                                                                                                                                       \\
% \midrule
%                     & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-7}                    
%                     & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
% \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
% caltech256          & -0.6±0.1                   & -0.1±0.0                   & -0.2±0.2                   & -0.0±0.1                   & -0.0±0.1                       & 3.7±1.9                       \\
% cifar10             & inf                        & inf                        & 0.4±0.7                    & 0.5±0.6                    & 0.5±0.6                        & 2.3±1.9                       \\
% cifar100            & 0.2±0.7                    & 0.3±0.6                    & -0.6±0.2                   & 0.0±0.0                    & -0.1±1.2                       & 4.7±0.5                       \\
% cub200              & -0.1±0.1                   & -0.1±0.0                   & -0.3±0.0                   & -0.0±0.0                   & -0.0±0.0                       & 4.3±0.9                       \\
% decathlon\_aircraft & inf                        & inf                        & 13.3±11.4                  & 13.3±11.4                  & 0.2±0.0                        & 3.7±0.5                       \\
% decathlon\_dtd      & 0.7±0.4                    & 0.7±0.4                    & 3.1±1.2                    & 3.1±1.2                    & 1.3±1.3                        & 1.7±0.9                       \\
% decathlon\_flowers  & -0.0±0.0                   & 0.0±0.0                    & 0.3±0.1                    & 0.3±0.1                    & 0.3±0.1                        & 1.3±0.5                       \\
% decathlon\_ucf101   & 18.8±12.4                  & 18.8±12.4                  & 0.6±0.6                    & 0.6±0.5                    & -0.1±0.1                       & 4.7±0.5                       \\
% eurosat             & inf                        & inf                        & -0.7±0.1                   & 0.0±0.1                    & 0.0±0.1                        & 3.3±1.2                       \\
% fgvc\_aircrafts     & inf                        & inf                        & inf                        & inf                        & 1.0±1.0                        & 2.0±0.8                       \\
% icassava            & 1.7±3.3                    & 1.7±3.3                    & inf                        & inf                        & 0.5±1.4                        & 3.7±1.9                       \\
% mit67               & 0.1±0.6                    & 0.3±0.4                    & 0.6±1.2                    & 0.8±1.1                    & 0.1±0.1                        & 3.0±0.8                       \\
% oxfordflowers       & 0.1±0.2                    & 0.2±0.1                    & 0.1±0.2                    & 0.2±0.1                    & 0.2±0.1                        & 2.3±1.9                       \\
% pets                & -0.8±0.0                   & -0.4±0.2                   & -0.8±0.0                   & -0.1±0.0                   & -0.2±0.1                       & 5.0±0.0                       \\
% stanfordcars        & 8.4±1.8                    & 8.4±1.8                    & 15.5±10.2                  & 15.5±10.2                  & 0.2±0.2                        & 3.0±0.0                       \\
% stanforddogs        & -0.3±0.4                   & -0.0±0.2                   & -0.3±0.2                   & -0.1±0.1                   & -0.1±0.0                       & 5.0±0.0                       \\
% \bottomrule
% \toprule
% \multicolumn{7}{c}{DETECTION}                                                                                                                                                                            \\
% \midrule
%                     & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-7}                     
%                     & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
% \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}                    
% cityscapes          & 0.4±0.8                    & 0.6±0.7                    & 0.1±0.4                    & 0.4±0.3                    & 0.4±0.3                        & 2.7±1.7                       \\
% comic               & inf                        & inf                        & 2.4±2.7                    & 2.7±2.4                    & 2.7±2.5                        & 2.3±1.9                       \\
% crowdhuman          & 5.5±7.2                    & 5.5±7.2                    & 1.0±1.5                    & 1.1±1.4                    & 1.1±1.4                        & 1.3±0.5                       \\
% duo                 & 1.7±0.7                    & 1.7±0.7                    & 0.8±1.0                    & 0.8±0.9                    & 0.1±0.2                        & 3.3±1.2                       \\
% kitti               & 5.0±6.3                    & 5.0±6.3                    & 0.2±0.4                    & 0.4±0.2                    & 0.2±0.2                        & 2.3±1.9                       \\
% minneapple          & -0.3±0.7                   & -0.0±0.6                   & -0.6±0.2                   & -0.2±0.2                   & 0.0±0.5                        & 4.3±0.9                       \\
% sixray              & 4.0±1.9                    & 4.0±1.9                    & -0.2±0.2                   & -0.0±0.0                   & -0.0±0.0                       & 5.0±0.0                       \\
% table               & 0.4±0.7                    & 0.5±0.7                    & 0.6±0.8                    & 0.7±0.7                    & -0.0±0.3                       & 4.3±0.9                       \\
% visdrone2019        & 0.0±0.0                    & 0.0±0.0                    & -0.3±0.1                   & -0.1±0.0                   & -0.1±0.0                       & 5.0±0.0                       \\
% watercolor          & 6.5±2.9                    & 6.5±2.9                    & 1.9±1.8                    & 1.9±1.7                    & -0.1±0.4                       & 4.0±1.4                      \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/data_fewshot_cls.tex <==
\begin{table*}[t!]
\rowcolors{2}{gray!10}{white}
\small
\centering
\caption{Estimating data requirements from few-shot to high-shot for classification tasks.}
\label{T:data_fewshot_classification}
\begin{tabular}{l|rr|rrrr}
\toprule
\multicolumn{7}{c}{CLASSIFICATION}                                                                                                                                                                       \\
\midrule
                    & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7}                    
                    & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
\caltech          & -0.6±0.1                   & -0.1±0.0                   & -0.2±0.2                   & -0.0±0.1                   & -0.0±0.1                       & 3.7±1.9                       \\
\cifar             & inf                        & inf                        & 0.4±0.7                    & 0.5±0.6                    & 0.5±0.6                        & 2.3±1.9                       \\
\cifarh            & 0.2±0.7                    & 0.3±0.6                    & -0.6±0.2                   & 0.0±0.0                    & -0.1±1.2                       & 4.7±0.5                       \\
\cub              & -0.1±0.1                   & -0.1±0.0                   & -0.3±0.0                   & -0.0±0.0                   & -0.0±0.0                       & 4.3±0.9                       \\
\daircraft & inf                        & inf                        & 13.3±11.4                  & 13.3±11.4                  & 0.2±0.0                        & 3.7±0.5                       \\
\ddtd      & 0.7±0.4                    & 0.7±0.4                    & 3.1±1.2                    & 3.1±1.2                    & 1.3±1.3                        & 1.7±0.9                       \\
\dflowers  & -0.0±0.0                   & 0.0±0.0                    & 0.3±0.1                    & 0.3±0.1                    & 0.3±0.1                        & 1.3±0.5                       \\
\ducf101   & 18.8±12.4                  & 18.8±12.4                  & 0.6±0.6                    & 0.6±0.5                    & -0.1±0.1                       & 4.7±0.5                       \\
\eurosat             & inf                        & inf                        & -0.7±0.1                   & 0.0±0.1                    & 0.0±0.1                        & 3.3±1.2                       \\
\fgvcaircrafts     & inf                        & inf                        & inf                        & inf                        & 1.0±1.0                        & 2.0±0.8                       \\
\icassava            & 1.7±3.3                    & 1.7±3.3                    & inf                        & inf                        & 0.5±1.4                        & 3.7±1.9                       \\
\mit               & 0.1±0.6                    & 0.3±0.4                    & 0.6±1.2                    & 0.8±1.1                    & 0.1±0.1                        & 3.0±0.8                       \\
\oxfordflowers       & 0.1±0.2                    & 0.2±0.1                    & 0.1±0.2                    & 0.2±0.1                    & 0.2±0.1                        & 2.3±1.9                       \\
\pets                & -0.8±0.0                   & -0.4±0.2                   & -0.8±0.0                   & -0.1±0.0                   & -0.2±0.1                       & 5.0±0.0                       \\
\stanfordcars        & 8.4±1.8                    & 8.4±1.8                    & 15.5±10.2                  & 15.5±10.2                  & 0.2±0.2                        & 3.0±0.0                       \\
\stanforddogs        & -0.3±0.4                   & -0.0±0.2                   & -0.3±0.2                   & -0.1±0.1                   & -0.1±0.0                       & 5.0±0.0                       \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/data_fewshot_det.tex <==
\begin{table*}[t!]
\rowcolors{2}{gray!10}{white}
\small
\centering
\caption{Estimating data requirements from few-shot to high-shot for detection tasks.}
\label{T:data_fewshot_detection}
\begin{tabular}{l|rr|rrrr}
\toprule
\multicolumn{7}{c}{DETECTION}                                                                                                                                                                            \\
\midrule
                    & \multicolumn{2}{c}{\textbf{powerlaw}}                            & \multicolumn{4}{c}{\textbf{piecewise}}                                                                                            \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7}                     
                    & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{1 step} & \multicolumn{1}{c}{5 step} & \multicolumn{1}{c}{5 step 5\%} & \multicolumn{1}{c}{avg steps} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}                    
\cityscapes          & 0.4±0.8                    & 0.6±0.7                    & 0.1±0.4                    & 0.4±0.3                    & 0.4±0.3                        & 2.7±1.7                       \\
\comic               & inf                        & inf                        & 2.4±2.7                    & 2.7±2.4                    & 2.7±2.5                        & 2.3±1.9                       \\
\crowdhuman          & 5.5±7.2                    & 5.5±7.2                    & 1.0±1.5                    & 1.1±1.4                    & 1.1±1.4                        & 1.3±0.5                       \\
\duo                 & 1.7±0.7                    & 1.7±0.7                    & 0.8±1.0                    & 0.8±0.9                    & 0.1±0.2                        & 3.3±1.2                       \\
\kitti               & 5.0±6.3                    & 5.0±6.3                    & 0.2±0.4                    & 0.4±0.2                    & 0.2±0.2                        & 2.3±1.9                       \\
\minneapple          & -0.3±0.7                   & -0.0±0.6                   & -0.6±0.2                   & -0.2±0.2                   & 0.0±0.5                        & 4.3±0.9                       \\
\sixray              & 4.0±1.9                    & 4.0±1.9                    & -0.2±0.2                   & -0.0±0.0                   & -0.0±0.0                       & 5.0±0.0                       \\
\table               & 0.4±0.7                    & 0.5±0.7                    & 0.6±0.8                    & 0.7±0.7                    & -0.0±0.3                       & 4.3±0.9                       \\
\visdrone        & 0.0±0.0                    & 0.0±0.0                    & -0.3±0.1                   & -0.1±0.0                   & -0.1±0.0                       & 5.0±0.0                       \\
\watercolor          & 6.5±2.9                    & 6.5±2.9                    & 1.9±1.8                    & 1.9±1.7                    & -0.1±0.4                       & 4.0±1.4                      \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/perf_fewshot.tex <==
\begin{table*}[ht]
\rowcolors{2}{gray!10}{white}
\centering
\caption{Estimating performance from few-shot to high-shot}
\label{T:performance_fewshot}
\begin{tabular}{lrrrrrr}
\toprule
\multicolumn{7}{c}{CLASSIFICATION}                                                                                                                                       \\
\midrule
                    & \multicolumn{1}{l}{\textbf{powerlaw}} & \textbf{algebraic} & \textbf{arctan}  & \textbf{logarithmic} & \textbf{piecewise} & \textbf{piecewise ub} \\
% \cmidrule(lr){2-7}
\caltech          & 10.3±3.6                              & 9.1±5.3            & 3.0±1.5          & 12.3±3.5             & \textbf{2.0±0.9}   & 1.2±0.5               \\
\cifar             & 6.7±2.2                               & 7.6±3.3            & 6.0±6.2          & 5.2±0.1              & \textbf{0.9±0.5}   & 0.5±0.4               \\
\cifarh            & 6.5±3.1                               & 22.5±0.1           & 17.2±7.3         & 22.2±0.4             & \textbf{6.1±3.5}   & 5.3±3.8               \\
\cub              & \textbf{2.6±0.3}                               & 18.5±0.9           & 14.1±3.9         & 16.8±1.3             & 4.0±0.1   & 0.7±0.1               \\
\daircraft & 18.0±1.8                              & 17.8±13.8          & 23.5±15.9        & 11.5±2.1             & \textbf{11.1±4.2}  & 11.1±4.1              \\
\ddtd      & 3.2±1.9                               & 5.3±1.2            & 4.7±2.5          & \textbf{3.2±0.9}     & 5.6±1.7            & 2.1±1.1               \\
\dflowers  & \textbf{1.0±0.3}                      & 1.1±0.4            & 1.5±0.3          & 1.2±0.5              & 2.0±0.3            & 1.1±0.0               \\
\ducf   & 14.5±1.9                              & 16.5±14.6          & 15.5±4.9         & 12.3±10.7            & \textbf{4.1±3.0}   & 4.1±2.9               \\
\eurosat             & 2.6±0.6                               & 4.3±3.2            & 4.2±2.4          & 2.1±0.2              & \textbf{0.9±0.2}   & 0.9±0.2               \\
\fgvcaircrafts     & 25.8±1.6                              & 18.1±2.4           & \textbf{9.2±7.4} & 10.5±6.7             & 19.1±1.4           & 11.1±1.8              \\
\icassava            & 9.2±6.7                               & 12.4±7.9           & 14.6±4.8         & 12.2±6.6             & \textbf{6.9±2.4}   & 6.9±2.4               \\
\mitd               & \textbf{4.2±1.7}                      & 15.8±6.4           & 8.2±5.3          & 11.7±6.5             & 4.3±2.5            & 3.9±2.3               \\
\oxfordflowers       & 1.5±0.4                               & 1.6±0.2            & 1.5±0.3          & 1.4±0.5              & \textbf{1.2±0.3}   & 1.1±0.4               \\
\pets                & 9.2±0.4                               & 8.4±0.7            & \textbf{1.1±0.5} & 9.7±0.2              & 5.6±0.8            & 1.7±0.5               \\
\stanfordcars        & 26.4±1.3                              & 18.8±0.4           & 17.6±2.9         & \textbf{14.2±0.6}    & 17.3±2.7           & 7.7±3.3               \\
\stanforddogs        & 6.1±5.4                               & 5.2±3.1            & 7.8±2.7          & 12.5±2.1             & \textbf{2.3±1.0}   & 1.2±0.1               \\
\rowcolor{gray!20}
MEAN                & 9.2±2.1                               & 11.4±4.0           & 9.3±4.3          & 9.9±2.7              & \textbf{5.8±1.6}   & 3.8±1.5               \\
\bottomrule
\toprule
\multicolumn{7}{c}{DETECTION}                                                                                                                                           \\
\midrule
\rowcolor{white}
         & \multicolumn{1}{l}{\textbf{powerlaw}} & \textbf{algebraic} & \textbf{arctan}  & \textbf{logarithmic} & \textbf{piecewise} & \textbf{piecewise ub} \\
cityscapes   & 1.3±0.8                               & 1.2±0.5            & 1.5±0.6          & 1.1±0.8              & \textbf{1.1±0.5}   & 0.9±0.6               \\
comic        & 4.4±2.9                               & 10.0±6.3           & 28.0±33.9        & \textbf{3.9±1.7}     & 4.1±1.0            & 3.4±2.0               \\
crowdhuman   & 0.8±0.2                               & 1.0±0.2            & 1.5±0.5          & 0.8±0.1              & \textbf{0.7±0.3}   & 0.5±0.3               \\
duo          & 3.9±1.8                               & 5.9±4.4            & 4.5±1.6          & 2.9±2.2              & \textbf{2.4±0.5}   & 1.8±0.9               \\
kitti        & 2.6±2.1                               & 3.3±2.0            & \textbf{1.5±1.0} & 2.2±1.1              & 1.6±0.7            & 1.5±1.4               \\
minneapple   & 4.7±2.3                               & 1.2±0.5            & \textbf{1.1±0.3} & 1.3±0.6              & 1.9±1.0            & 0.6±0.1               \\
sixray       & 6.9±0.9                               & 28.3±17.7          & 8.3±9.9          & 9.6±9.9              & \textbf{2.7±2.7}   & 2.4±1.1               \\
table        & 5.9±2.7                               & 8.5±5.1            & 7.8±2.2          & 6.3±3.7              & \textbf{5.5±0.8}   & 5.5±2.2               \\
visdrone2019 & \textbf{0.3±0.1}                      & 1.0±0.4            & 0.7±0.3          & 0.9±0.3              & 0.8±0.3            & 0.4±0.1               \\
watercolor   & 5.2±1.5                               & 19.4±22.1          & 6.7±2.7          & 6.7±3.0              & \textbf{3.2±1.4}   & 3.1±1.7               \\
\rowcolor{gray!20}
MEAN         & 3.6±1.5                               & 8.0±5.9            & 6.2±5.3          & 3.6±2.3              & \textbf{2.4±0.9}   & 2.0±1.0               \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/perf_fewshot_rebuttal.tex <==
\begin{table}[t]
\rowcolors{2}{gray!10}{white}
\footnotesize
\centering
\caption{Out-of-distribution vs in-distribution meta-model.}
\label{T:perf_fewshot_rebuttal}
\begin{tabular}{lrrr}
\toprule
                    & powerlaw             & piecewise   & piecewise \\
                    & \multicolumn{1}{l}{} & out-of-dist & in-dist   \\
\midrule                    
\caltech          & 2.9±2.2              & 1.1±0.8     & 1.2±0.9   \\
\cifar             & 18.9±2.2             & 1.9±1.4     & 1.9±1.4   \\
\cifarh            & 15.1±0.1             & 11.8±0.9    & 0.9±0.1   \\
\cub              & 4.9±1.5              & 4.0±1.6     & 1.7±1.2   \\
\daircraft & 20.3±0.6             & 10.6±1.1    & 10.7±1.1  \\
\ddtd      & 5.6±3.0              & 5.4±1.3     & 6.1±3.3   \\
\dflowers  & 2.0±1.1              & 2.6±0.7     & 2.1±0.7   \\
\ducf   & 15.0±1.0             & 3.5±1.9     & 3.5±2.1   \\
\eurosat             & 4.8±4.3              & 0.3±0.1     & 0.3±0.1   \\
\fgvcaircrafts     & 26.6±1.8             & 15.2±5.0    & 9.4±1.9   \\
\icassava            & 14.3±5.8             & 1.8±0.7     & 1.8±0.7   \\
\mitd               & 7.7±2.2              & 5.9±2.9     & 2.1±0.9   \\
\oxfordflowers       & 1.5±1.0              & 1.1±0.4     & 1.1±0.4   \\
\pets                & 4.1±2.8              & 2.0±0.5     & 2.4±0.2   \\
\stanfordcars        & 23.9±1.1             & 14.7±1.4    & 7.6±1.5   \\
\stanforddogs        & 8.7±3.1              & 6.8±0.5     & 7.1±0.5   \\
\midrule
AVERAGE             & 11.0±2.1             & 5.5±1.3     & 3.7±1.1   \\
\bottomrule
\end{tabular}
\end{table}

==> tables/predictors.tex <==
\begin{table*}[!t]
\centering
\caption{Choice of predictors for performance estimation.}
\label{T:predictors}
% \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcl}
         \toprule
         predictor & \# params & $\log(1-\hat{v}(n;\bm{\theta}))$ \\
         \midrule
         power law (linear) & 2 & $\theta_1 + \theta_2 \log(n)$ \\
         power law ~\cite{cortes1993learning} & 3 & $\log\left(\theta_1 n^{\theta_2} + \theta_3\right)$ \\
         arctan~\cite{mahmood2022much} & 3 &  $\log\left(-\frac{200}{\pi} \arctan(\theta_1 \frac{\pi}{2}  n + \theta_2) + \theta_3\right)$ \\
         logarithmic~\cite{mahmood2022much} & 3 & $\log\left(\theta_1 \log(n + \theta_2) + \theta_3\right)$ \\
         algebraic~\cite{mahmood2022much} & 3 & $\log\left(-\frac{100  n}{ (1 + | \theta_1 n |^{\theta_2})^{1/\theta_2}}  + \theta_3\right)$ \\
         \midrule
         piecewise (ours) & 4 & $\begin{cases}
            \theta_1 + \theta_2 \log(n) + \theta_3 \log(n)^2,& \text{if } n\leq N \\
            \theta_4 + \theta_5 \log(n),              & \text{otherwise}
            \end{cases}$ \\
         \bottomrule
    \end{tabular}
% }
\end{table*}
